Self-similar orbit-averaged Fokker-Planck equation for isotropic spherical dense clusters (i) accurate pre-collapse solution

This is the first paper of a series of our works on the self-similar orbit-averaged Fokker-Planck (OAFP) equation for distribution function of stars in dense isotropic star clusters. At the late stage of relaxation evolution of the clusters, standard stellar dynamics predicts that the clusters evolve in a self-similar fashion forming collapsing cores. However, the corresponding mathematical model, the self-similar OAFP equation, has never been solved on the whole energy domain $(-1< E < 0)$. The existing works based on kinds of finite difference methods provide solutions only on the truncated domain $-1< E<-0.2$. To broaden the range of the truncated domain, the present work resorts to a (highly accurate and efficient) Gauss-Chebyshev pseudo-spectral method. We provide a spectral solution, whose number of significant figures is four, on the whole domain. Also, the solution can reduce to a semi-analytical form whose degree of polynomials is only eighteen holding three significant figures. We also provide the new eigenvalues; $c_{1}=9.0925\times10^{-4}$, $c_{2}=1.1118\times10^{-4}$, $c_{3}=7.1975\times10^{-2}$ and $c_{4}=3.303\times10^{-2}$, corresponding to the core collapse rate $\xi=3.64\times10^{-3}$, scaled escape energy $\chi_\text{esc}=13.881$ and power-law exponent $\alpha=2.2305$. Since the solution on the whole domain is unstable against degree of Chebyshev polynomials, we also provide spectral solutions on truncated domains ( $-1< E<E_\text{max}$, where $-0.35<E_\text{max}<-0.03$) to explain how to handle the instability. By reformulating the OAFP equation in several ways, we improve the accuracy of the spectral solution and reproduce an existing self-similar solution, which infers that existing solutions have only one significant figure at best.

==> Section5_old__Result_trunc.tex <==
\section{Self-similar solution on truncated domain(OLD)}\label{sec:domain_trunc}

\hspace{0.6cm}Since the whole-domain solution is unstable against change in degrees of polynomials and the present work relies on a collocation method, it is imperative to construct a spectral solution whose accuracy is less sensitive to change in degrees of polynomials. According to the results for the whole-domain solution (Section \ref{sec:ss_soln_whole}), the regularized DF $\varv_{F}(x)$ may be extrapolated by the power-law functions $\varv_{F}^{\text{(ex)}}(x)$, equation \eqref{Eq.vF_extrap}, approximately at a point on the domain $-0.02\lesssim E \lesssim -0.2$ (or $-0.96\lesssim x\lesssim-0.6$) on which the regularized solutions behave as constant functions of $x$.


  The domain-truncated solutions are shown in Table \ref{table:trunc_soln} in which the maximum significant figures of the eigenvalue $\beta$ is limited  up to 10, \footnote{The condition number of the Jacobian in the iteration process is of the order of $10^{7}$, meaning one can obtain approximately five significant-figure solution since the minimum of the precision is to be considered to of the order of $10^{-12}$. Considering, the gap between $c_{1}$ (or $\beta$) and $c_{4}$ in accuracy is of the order of $10^{-5}$, 10 digit significant figure is moderate choice for $\beta$.} and only the values of $\mid1-c_{1}/c_{1\text{o}}\mid$, $\mid1-c^{*}_{4}/c^{*}_{4\text{o}}\mid$ and $\varv_{I}(x=1)$ are presented to show the accuracy of solutions. The truncated-domain solution is advantage over the whole solution in sense that the low degrees $25\sim55$ of polynomials are needed to make Newton iteration work; even the lower degrees shows a good result in accuracy for $c^{*}_{4}$ which was the least accuracy in the whole-domain solution.Yet, Newton iteration worked still limited degrees of polynomials.

\begin{table*}[h]\large
	\ra{1.3}
	\scalebox{0.7}{
	\begin{tabular}{@{}clccc@{}}
             \large{$E_\text{min}=-0.03$} & \multicolumn{2}{l}{\large{or $\quad (-E_\text{min})^{\beta}\approx 3.5\times10^{-13}$}}   &  &  \\
              \toprule
		 \large{$N$} & Eigenvalue $\beta$ & $\mid1-c_{1}/c_{1\text{o}} \mid$ &  $\mid1-c^{*}_{4}/c^{*}_{4\text{o}} \mid$  & $\varv_{I}(x=1)$  \\ 
		\midrule
             $55$ & $8.178371160$ & $6.5\times10^{-10}$& $2.6\times10^{-6}$  &$ 1.6\times10^{-8}$\\
		$50$ & $8.178371160$ & $7.1\times10^{-10}$& $2.9\times10^{-6}$  &$ 1.7\times10^{-8}$\\
		$40$ & $8.178371165$ & $2.4\times10^{-9}$& \underline{$6.9\times10^{-7}$}  &\underline{$ 4.3\times10^{-9}$}\\
		$30$ & $8.178370376$ & $1.3\times10^{-7}$& $9.8\times10^{-6}$  & $8.1\times10^{-10}$\\
		$25$ & $8.1783436$ & $8.1\times10^{-7}$& $1.3\times10^{-4}$  & $1.1\times10^{-9}$\\
		\bottomrule
	\end{tabular}}
	\scalebox{0.7}{
	\begin{tabular}{@{}clccc@{}}
             \large{$E_\text{min}=-0.04$} & \multicolumn{2}{l}{\large{or $\quad (-E_\text{min})^{\beta}\approx 3.7\times10^{-12}$}}   &  &  \\
              \toprule
		 \large{$N$} & Eigenvalue $\beta$ & $\mid1-c_{1}/c_{1\text{o}} \mid$ &  $\mid1-c^{*}_{4}/c^{*}_{4\text{o}} \mid$  & $\varv_{I}(x=1)$  \\ 
		\midrule
             $55$ & $8.178371160$ & $5.1\times10^{-10}$& $2.1\times10^{-6}$  &$ 1.3\times10^{-8}$\\
		$50$ & $8.178371160$ & $1.9\times10^{-10}$& $8.3\times10^{-7}$  &$ 5.1\times10^{-9}$\\
		$40$ & $8.178371170$ & $1.4\times10^{-10}$& \underline{$7.1\times10^{-7}$}  &\underline{$ 4.0\times10^{-9}$}\\
		$30$ & $8.17837159$ & $1.8\times10^{-7}$& $4.7\times10^{-6}$  & $6.7\times10^{-9}$\\
		$25$ & $8.1783585$ & $1.7\times10^{-6}$& $6.8\times10^{-5}$  & $5.2\times10^{-9}$\\
		\bottomrule
	\end{tabular}}\vspace{0.5cm}
\scalebox{0.7}{
\begin{tabular}{@{}clccc@{}}
             \large{$E_\text{min}=-0.05$} & \multicolumn{2}{l}{\large{or $\quad (-E_\text{min})^{\beta}\approx 2.2\times10^{-11}$}}  &   &  \\
              \toprule
		 \large{$N$} & Eigenvalue $\beta$ & $\mid1-c_{1}/c_{1\text{o}} \mid$ &  $\mid1-c^{*}_{4}/c^{*}_{4\text{o}} \mid$  & $\varv_{I}(x=1)$  \\ 
		\midrule
                     &                   &                                         &                                        &  \\
		$50$ & $8.178371158$ & $2.8\times10^{-9}$& $1.0\times10^{-5}$  &$ 6.8\times10^{-8}$\\
		$40$ & $8.178371165$ & $5.5\times10^{-9}$& \underline{$9.7\times10^{-7}$}  & \underline{$ 3.0\times10^{-9}$}\\
		$30$ & $8.1783723$ & $2.1\times10^{-8}$& $3.7\times10^{-6}$  & $3.1\times10^{-8}$\\
		$25$ & $8.178373$ & $1.5\times10^{-6}$& $1.9\times10^{-5}$  & $4.0\times10^{-9}$\\
		\bottomrule
	\end{tabular}}
\scalebox{0.7}{
\begin{tabular}{@{}clccc@{}}
             \large{$E_\text{min}=-0.06$} & \multicolumn{2}{l}{\large{or $\quad (-E_\text{min})^{\beta}\approx 1.0\times10^{-10}$}} &                                     &  \\
              \toprule
		 \large{$N$} & Eigenvalue $\beta$ & $\mid1-c_{1}/c_{1\text{o}} \mid$ &  $\mid1-c^{*}_{4}/c^{*}_{4\text{o}} \mid$  & $\varv_{I}(x=1)$  \\ 
		\midrule
		$40$ & $8.178371160$ & $8.3\times10^{-10}$& \underline{$8.7\times10^{-7}$}  & \underline{$ 2.2\times10^{-9}$}\\
		$30$ & $8.17837225$ & $1.5\times10^{-7}$& $5.0\times10^{-6}$  & $8.1\times10^{-9}$\\
		$25$ & $8.1783813$ & $2.4\times10^{-7}$& $1.6\times10^{-5}$  & $2.3\times10^{-9}$\\
		\bottomrule
	\end{tabular}}
\scalebox{0.7}{
\begin{tabular}{@{}clccc@{}}
             \large{$E_\text{min}=-0.07$} & \multicolumn{2}{l}{\large{or $\quad (-E_\text{min})^{\beta}\approx 3.6\times10^{-10}$}}                                 &   &  \\
              \toprule
		 \large{$N$} & Eigenvalue $\beta$ & $\mid1-c_{1}/c_{1\text{o}} \mid$ &  $\mid1-c^{*}_{4}/c^{*}_{4\text{o}} \mid$  & $\varv_{I}(x=1)$  \\ 
		\midrule
		$35$ & $8.178371159$ & $8.6\times10^{-9}$& \underline{$2.3\times10^{-6}$}  & \underline{$ 1.4\times10^{-9}$}\\
		$30$ & $8.1783717$ & $2.2\times10^{-7}$& $1.9\times10^{-5}$  & $9.7\times10^{-8}$\\
		$25$ & $8.178382$ & $1.1\times10^{-6}$& $5.0\times10^{-5}$  & $9.8\times10^{-8}$\\
		\bottomrule
	\end{tabular}}
\scalebox{0.7}{
\begin{tabular}{@{}clccc@{}}
             \large{$E_\text{min}=-0.08$} & \multicolumn{2}{l}{\large{or $\quad (-E_\text{min})^{\beta}\approx 1.1\times10^{-9}$}}    &     &  \\
              \toprule
		 \large{$N$} & Eigenvalue $\beta$ & $\mid1-c_{1}/c_{1\text{o}} \mid$ &  $\mid1-c^{*}_{4}/c^{*}_{4\text{o}} \mid$  & $\varv_{I}(x=1)$  \\ 
		\midrule
		$25$ & $8.1783768$ & $2.8\times10^{-6}$& $\underline{4.7\times10^{-5}}$  & \underline{$ 7.9\times10^{-9}$}\\
		\bottomrule
	\end{tabular}}
	\caption{The numerical results for the truncated-domain formulation at $x_\text{min}=-0.9$ and $L=1$. $c_{1\text{o}}=9.09254120455\times10^{-4}$ and $c^{*}_{4\text{o}}=3.03155222\times10^{-1}$. The minimum values of $\mid1-c^{*}_{4}/c^{*}_{4\text{o}}\mid$ and $\varv_{I}(x=1)$ are underlined to highlight the accuracy for each $N$. The results do not include some data in which the value of $\varv_{I}(x=1)$ is greater than of the order of $\sim10^{-7}$. for convenience The Newton iteration method was very hard to converge for $N<25$ and the degrees above the maximum values of $N$ for each $E_\text{min}$, and the change in new $\{a_{n}\}$ and old one was reduced to $\sim10^{-6}$ or diverged while the data in the table are the result when the change reached of the order of $\sim10^{-12}$.}
	\label{table:trunc_soln}
\end{table*}

   To see the relationship between truncated-domain solution and truncated-domain solution, the eigenvalue $\beta$ is set to the reference value $\beta_{\text{o}}$ and solution was recalculated at $x_\text{min}=-0.94$ at which the relative deviation of the whole-domain solution from the asymptote reaches of the order of $10^{-12}$. The figures corresponding to Figures \ref{fig:Stab_Deg} and \ref{fig:Del_asymFKGL} are shown in Figures \ref{fig:Del_asymFKGL_N400_trunc} and \ref{fig:Stab_Deg_c4vKcond_trunc}. The former shows that the truncated-domain solution for $N=400$ does not show diverging behavior as $E\to0$ in the relative deviation of the solutions from the asymptotes. Also, Table \ref{fig:Stab_Deg_c4vKcond_trunc} shows that the stability of eigenvalues and solution against change in degree is ideal; as the degree $N$ increases, the solution approaches a specific function and the eigenvalues converge to the reference values increasing the accuracy from of the order of $10^{-7}$ to $10^{-7}$. 




\begin{figure}[h]
	\centering
\tikzstyle{every node}=[font=\Large]
	\begin{tikzpicture}[scale=0.7]
	\begin{loglogaxis}[width=5cm, height=10cm, grid=major,xlabel=\Large{$-E$},title=\Large{$\mid(1-F(E)/F_\text{asy}(E)\mid$},xmin=1e-3,xmax=1,ymin=1e-14,ymax=1e4, legend pos=north east]
	\addplot [color = bred,mark=no,thick,solid] table[x index=0, y index=1]{Del_asymFKGL_400_trunc.txt}; 
 \addlegendentry{\large{tuncated}}
\addplot [color = blue,mark=no,thick,dashed] table[x index=0, y index=1]{Del_asymFKGL_400.txt}; 
\addlegendentry{\large{whole}}
	\end{loglogaxis}
	\end{tikzpicture}
\begin{tikzpicture}[scale=0.7]
	\begin{loglogaxis}[width=5cm, height=10cm, grid=major,xlabel=\large{$-E$},title=\Large{$\mid(1-I(E)/I_\text{asy}(E)\mid$},xmin=1e-3,xmax=1,ymin=1e-13,ymax=1e4, legend pos=north east]
	\addplot [color = bred ,mark=no,thick,solid ] table[x index=0, y index=2]{Del_asymFKGL_400_trunc.txt}; 
 \addlegendentry{\large{tuncated}}
\addplot [color = blue,mark=no,thick,dashed] table[x index=0, y index=2]{Del_asymFKGL_400.txt}; 
      \addlegendentry{\large{whole}}
	\end{loglogaxis}
	\end{tikzpicture}
\begin{tikzpicture}[scale=0.7]
	\begin{loglogaxis}[width=5cm, height=10cm, grid=major,xlabel=\Large{$-E$},title=\Large{$\mid(1-G(E)/G_\text{asy}(E)\mid$},xmin=1e-3,xmax=1,ymin=1e-13,ymax=1e4, legend pos=north east]
	\addplot [color = bred ,mark=no,thick,solid] table[x index=0, y index=3]{Del_asymFKGL_400_trunc.txt}; 
 \addlegendentry{\large{tuncated}}
\addplot [color = blue,mark=no,thick,dashed] table[x index=0, y index=3]{Del_asymFKGL_400.txt}; 
      \addlegendentry{\large{whole}}
	\end{loglogaxis}
	\end{tikzpicture}
	\centering
	\begin{tikzpicture}[scale=0.7]
	\begin{loglogaxis}[width=5cm, height=10cm, grid=major,xlabel=\Large{$-E$},title=\Large{$\mid(1-J(E)/J_\text{asy}(E)\mid$},xmin=1e-3,xmax=1,ymin=1e-13,ymax=1e4, legend pos=north east]
	\addplot [color = bred ,mark=no,thick,solid] table[x index=0, y index=4]{Del_asymFKGL_400_trunc.txt}; 
 \addlegendentry{\large{tuncated}}
\addplot [color = blue,mark=no,thick,dashed] table[x index=0, y index=4]{Del_asymFKGL_400.txt}; 
      \addlegendentry{\large{whole}}
	\end{loglogaxis}
	\end{tikzpicture}
\caption{The relative deviations of the truncated ss-OAFP solutions from their own asymptotes on the whole- and truncated- domains ($N=400$, $F_\text{BC}=1$, $L=1$). The end point $x_\text{min}$ of the truncated domain is $-0.94$ i.e. $E_\text{min}=-0.03$.  }
\label{fig:Del_asymFKGL_N400_trunc}
\end{figure}



    \begin{figure}[h]
	\centering
	\tikzstyle{every node}=[font=\Large]
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[width=5cm,height=10cm, grid=major,xlabel=\Large{degree $N$},xmin=20,xmax=4.2e2,ymin=1e-13,ymax=1e-0, legend pos=north east]
	\addplot [color = bgreen ,mark=*, thick] table[x index=0, y index=1]{Stab_Deg_vKcond_trunc.txt}; 
     \addlegendentry{\large{$\varv_{I}(x=1)$}}
     \addplot [color = bred ,mark=square, thick] table[x index=0, y index=3]{Stab_Deg_vKcond_trunc.txt}; 
     \addlegendentry{$\mid1-c^{*}_{4}/c^{*}_{4\text{o}}\mid$}
      \end{semilogyaxis}
	\end{tikzpicture}\hspace{0.1cm}
		\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[width=5cm,height=10cm, grid=major,xlabel=\Large{degree $N$},title=\Large{Condition number},xmin=20,xmax=4.2e2,ymin=1e2,ymax=1e10, legend pos=north east]
	\addplot [color = bred ,mark=*, thick] table[x index=0, y index=2]{Stab_Deg_vKcond_trunc.txt}; 
	\end{semilogyaxis}
	\end{tikzpicture}\hspace{0.1cm}
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[width=6cm,height=10cm,legend columns=2, grid=major,xlabel=\Large{$E$},title=\Large{$\mid1-F(E_{K})^{(65)}/F(E_{K})^{(N)}\mid$},xmin=-1.1,xmax=0.1,ymin=1e-13,ymax=1e1, legend pos=north west]
	\addplot [color = black ,mark=square,thick,solid ]  table[x index=0, y index=1]{Stab_Deg_F_trunc.txt}; 
       \addlegendentry{\large{$N=40$}}
      \addplot [color = black ,mark=+, thick, solid] table[x index=0, y index=2]{Stab_Deg_F_trunc.txt}; 
       \addlegendentry{\large{$N=80$}}
      \addplot [color = black ,mark=triangle, thick, solid] table[x index=0, y index=3]{Stab_Deg_F_trunc.txt}; 
       \addlegendentry{\large{$N=100$}}
      \addplot [color = bblue ,mark=no, thick,densely dashed] table[x index=0, y index=4]{Stab_Deg_F_trunc.txt}; 
       \addlegendentry{\large{$N=150$}}
%\addplot [color = bgold ,mark=triangle, thick] table[x index=0, y index=5]{Stab_Deg_F_trunc.txt}; 
   %    \addlegendentry{\large{$N=200$}}
\addplot [color = bgold ,mark=no, thick, solid] table[x index=0, y index=6]{Stab_Deg_F_trunc.txt}; 
       \addlegendentry{\large{$N=250$}}
%\addplot [color = bgreen ,mark=o, thick] table[x index=0, y index=7]{Stab_Deg_F_trunc.txt}; 
     %  \addlegendentry{\large{$N=300$}}
%\addplot [color = bblue ,mark=o, thick] table[x index=0, y index=8]{Stab_Deg_F_trunc.txt}; 
       %\addlegendentry{\large{$N=350$}}
\addplot [only marks, color = bred ,mark=*, thick] table[x index=0, y index=9]{Stab_Deg_F_trunc.txt}; 
       \addlegendentry{\large{$N=400$}}
      \end{semilogyaxis}
	\end{tikzpicture}
	\caption{(Left panel)The dependence of the difference between the eigenvalue $c_4$ and the reference value $c^{*}_{4\text{o}}(=3.03155225)$, boundary value $\varv_{I}(x=1)$ and (Middle panel) condition number of the Jacobian matrix on the degree $N$ of Chebyshev polynomials.  (Right panel) The change in solution at specified nodes with different degrees of Chebyshev Polynomials. ($L=1$ and $F_\text{BC}=1$)}
	\label{fig:Stab_Deg_c4vKcond_trunc}
\end{figure}


Around at $x_\text{min}=-0.94$, the same stability were confirmed and all of them were converged their own solutions over $N=150$. Since the present concern is whether the truncated-domain solution is compatible with the whole solution obtained for $N=70$ and $\beta=\beta_\text{o}$, the results are compared in Figure \ref{fig:xmin_vK_Del_c1c4_N200_trunc}. The eigenvalue $c^{*}_{4}$ and $\varv_{I}(x=1)$ are minimum at $x_\text{min}=-0.95$. The reason why the value of $x_\text{min}=-0.95$ is optimal is quite simple; at equation level of the 4ODEs, the second term and last term asymptotically reaches the following relation
\begin{align}
\text{(3rd term)/(2nd term)}=-c1\left(\frac{1+x}{2}\right)^{a}
\end{align} 
once equating the factor to the machine precision of MATLA eps$\approx2.220^{-16}$, one obtains $x_\text{min}\approx-9.503$. This implies that one can not solve the ss-OAFP equation outside the domain $-0.9503<x<1$ or $-0.02485<E<0$ due to the limit of numerical precision. Yet, one's concern is  
 





The truncated-domain solutions
\begin{figure}[h]
	\centering
\tikzstyle{every node}=[font=\Large]
	\begin{tikzpicture}[scale=0.9]
\begin{semilogyaxis}[grid=major,xlabel=\Large{$N$},xmin=0, xmax=50,ymin=1e-17,ymax=1e-0, legend pos=south west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{N_vK_Del_c1c4_cF_xmin_082_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{N_vK_Del_c1c4_cF_xmin_082_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{N_vK_Del_c1c4_cF_xmin_082_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
%\addplot [color = blue,mark=o,thick] table[x index=0, y index=4]{N_vK_Del_c1c4_cF_xmin_082_trunc.txt}; 
%\addlegendentry{\large{min. of $Fn$}}
\node[above,red] at (30,1e-3) {$x_\text{min}=-0.82$};
\end{semilogyaxis}
\end{tikzpicture}
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[grid=major,xlabel=\Large{$N$},xmin=0, xmax=50,ymin=1e-17,ymax=1e-0, legend pos=south west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{N_vK_Del_c1c4_cF_xmin_084_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{N_vK_Del_c1c4_cF_xmin_084_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{N_vK_Del_c1c4_cF_xmin_084_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
%\addplot [color = blue,mark=o,thick] table[x index=0, y index=4]{N_vK_Del_c1c4_cF_xmin_084_trunc.txt}; 
%\addlegendentry{\large{min. of $Fn$}}
\node[above,red] at (30,1e-3) {$x_\text{min}=-0.84$};
	\end{semilogyaxis}
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[grid=major,xlabel=\Large{$N$},xmin=0, xmax=50,ymin=1e-17,ymax=1e-0, legend pos=south west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{N_vK_Del_c1c4_cF_xmin_086_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{N_vK_Del_c1c4_cF_xmin_086_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{N_vK_Del_c1c4_cF_xmin_086_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
%\addplot [color = blue,mark=o,thick] table[x index=0, y index=4]{N_vK_Del_c1c4_cF_xmin_086_trunc.txt}; 
%\addlegendentry{\large{min. of $Fn$}}
\node[above,red] at (30,1e-3) {$x_\text{min}=-0.86$};
	\end{semilogyaxis}
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[grid=major,xlabel=\Large{$N$},xmin=0, xmax=50,ymin=1e-17,ymax=1e-0, legend pos=south west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{N_vK_Del_c1c4_cF_xmin_088_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{N_vK_Del_c1c4_cF_xmin_088_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{N_vK_Del_c1c4_cF_xmin_088_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
%\addplot [color = blue,mark=o,thick] table[x index=0, y index=4]{N_vK_Del_c1c4_cF_xmin_088_trunc.txt}; 
%\addlegendentry{\large{min. of $Fn$}}
\node[above,red] at (30,1e-3) {$x_\text{min}=-0.88$};
	\end{semilogyaxis}
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[grid=major,xlabel=\Large{$N$},xmin=0, xmax=60,ymin=1e-17,ymax=1e-0, legend pos=south west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{N_vK_Del_c1c4_cF_xmin_090_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{N_vK_Del_c1c4_cF_xmin_090_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{N_vK_Del_c1c4_cF_xmin_090_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
%\addplot [color = blue,mark=o,thick] table[x index=0, y index=4]{N_vK_Del_c1c4_cF_xmin_090_trunc.txt}; 
%\addlegendentry{\large{min. of $Fn$}}
\node[above,red] at (30,1e-3) {$x_\text{min}=-0.90$};
	\end{semilogyaxis}
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[grid=major,xlabel=\Large{$N$},xmin=0, xmax=70,ymin=1e-17,ymax=1e-0, legend pos=south west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{N_vK_Del_c1c4_cF_xmin_092_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{N_vK_Del_c1c4_cF_xmin_092_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{N_vK_Del_c1c4_cF_xmin_092_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
%\addplot [color = blue,mark=o,thick] table[x index=0, y index=4]{N_vK_Del_c1c4_cF_xmin_092_trunc.txt}; 
%\addlegendentry{\large{min. of $Fn$}}
\node[above,red] at (30,1e-3) {$x_\text{min}=-0.92$};
	\end{semilogyaxis}
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.9]
	\begin{semilogyaxis}[grid=major,xlabel=\Large{$N$},xmin=0, xmax=75,ymin=1e-17,ymax=1e-0, legend pos=south west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{N_vK_Del_c1c4_cF_xmin_094_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{N_vK_Del_c1c4_cF_xmin_094_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{N_vK_Del_c1c4_cF_xmin_094_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
%\addplot [color = blue,mark=o,thick] table[x index=0, y index=4]{N_vK_Del_c1c4_cF_xmin_094_trunc.txt}; 
%\addlegendentry{\large{min. of $Fn$}}
\node[above,red] at (30,1e-3) {$x_\text{min}=-0.94$};
	\end{semilogyaxis}
	\end{tikzpicture}
\caption{The relative deviation of the eigenvalues $c_{1}$ and $c^{*}_{4}$ from the reference values and the value of $\varv_{I}(x=1)$ against change in the degree $N$ for $L=1$ and $F_\text{BC}=1$. }
\label{N_vK_Del_c1c4_cF_trunc}
\end{figure}


The relative errors of the eigenvalues are shown in Figure \ref{Emin_vK_Del_c1c4_BETAo_trunc} for each of $x_\text{min}$.

    \begin{figure}[h]
	\centering
	\tikzstyle{every node}=[font=\Large]
	\begin{tikzpicture}[scale=0.8]
	\begin{loglogaxis}[width=6cm,height=10cm,grid=major,xlabel=\Large{$-E_\text{min}$},xmin=-0.96, xmax=-0.80,ymin=1e-17,ymax=1e-0, legend pos=north west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{Emin_vK_Del_c1c4_BETAo_trunc.txt}; 
\addlegendentry{\large{$\varv_{I}(x=1)$}}
\addplot [color = blue,mark=*,thick] table[x index=0, y index=2]{Emin_vK_Del_c1c4_BETAo_trunc.txt}; 
\addlegendentry{\large{$\mid1-c_{1}/ c_{1\text{o}}\mid$}}
\addplot [color = blue,mark=o,thick] table[x index=0, y index=3]{Emin_vK_Del_c1c4_BETAo_trunc.txt}; 
\addlegendentry{\large{$\mid1-c^{*}_{4}/ c^{*}_{4\text{o}}\mid$}}
 \addplot [color = blue,mark=no,thick,solid] table[x index=0, y index=4]{Emin_vK_Del_c1c4_BETAo_trunc.txt}; 
  \addlegendentry{\large{$c_{1\text{o}}(1/2+1/2)^{\beta_\text{o}}/c^{*}_{4\text{o}}$}}
 %\addplot [color = blue,mark=no,thick,dashed] table[x index=0, y index=5]{xmin_vK_Del_c1c4_N200_trunc.txt}; 
  %\addlegendentry{\large{eps}}
	\end{loglogaxis}
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.8]
	\begin{loglogaxis}[width=6cm,height=10cm,grid=major,xlabel=\Large{$-E_\text{min}$},xmin=-0.94, xmax=-0.001,ymin=1e-12,ymax=1e-8, legend pos=north west]
\addplot [color = bred,mark=square,thick,solid] table[x index=0, y index=1]{compari_N70_N65_xm094.txt}; 
	\end{loglogaxis}
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.8]
	\begin{semilogyaxis}[width=6cm,height=10cm,legend columns=2, grid=major,xlabel=\Large{$E$},title=\Large{$\mid1-F(E_{K})^{(65)}/F(E_{K})^{(N)}\mid$},xmin=0.01,xmax=1,ymin=1e-13,ymax=1e1, legend pos=north west]
	\addplot [color = black ,mark=square,thick,solid ]  table[x index=0, y index=1]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=25$}}
      \addplot [color = black ,mark=+, thick, solid] table[x index=0, y index=2]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=30$}}
      \addplot [color = black ,mark=triangle, thick, solid] table[x index=0, y index=3]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=35$}}
      \addplot [color = bblue ,mark=no, thick,densely dashed] table[x index=0, y index=4]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=40$}}
\addplot [color = bgold ,mark=triangle, thick] table[x index=0, y index=5]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=45$}}
\addplot [color = bgold ,mark=no, thick, solid] table[x index=0, y index=6]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=50$}}
\addplot [color = bgreen ,mark=o, thick] table[x index=0, y index=7]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=55$}}
\addplot [color = bblue ,mark=o, thick] table[x index=0, y index=8]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=60$}}
\addplot [only marks, color = bred ,mark=*, thick] table[x index=0, y index=9]{Stab_Deg_F_xmin_094_N65.txt}; 
       \addlegendentry{\large{$N=70$}}
      \end{semilogyaxis}
	\end{tikzpicture}
	\caption{(Left panel)The dependence of the difference between the eigenvalue $c_4$ and the reference value $c^{*}_{4\text{o}}(=3.03155225)$, boundary value $\varv_{I}(x=1)$ and (Middle panel) condition number of the Jacobian matrix on the degree $N$ of Chebyshev polynomials.  (Right panel) The change in solution at specified nodes with different degrees of Chebyshev Polynomials. ($L=1$ and $F_\text{BC}=1$)}
	\label{fig:Stab_Deg_F_xmin_094_N65}
\end{figure}


==> Section6_1_iteration.tex <==
\section{Why is Newton iteration method hard to work?}
The difficulty in numerical integration of the OAFP equation originates from the complicated structure of the 4ODEs. To understand the structure, one must refer to the value of the infinity norms of the Chebyshev coefficients associated to 4ODE;
\begin{align}
&\left\|\{F_n\}^\text{new}-\{F_n\}^\text{old}\right\|_{\infty}\sim\mathcal{O}\left(10^{-13}\right), \hspace{1cm}\left\|\{Q_n\}^\text{new}-\{Q_n\}^\text{old}\right\|_{\infty}\sim\mathcal{O}\left(10^{-14}\right)\\
&\left\|\{G_n\}^\text{new}-\{G_n\}^\text{old}\right\|_{\infty}\sim\left\|\{K_n\}^\text{new}-\{K_n\}^\text{old}\right\|_{\infty}\sim\left\|\{L_n\}^\text{new}-\{L_n\}^\text{old}\right\|_{\infty}\sim\mathcal{O}\left(10^{-16}\right)\sim eps.\\
&\left\|c_1^\text{new}-c_1^\text{old}\right\|_{\infty}\sim\sim\mathcal{O}\left(10^{-16}\right),\hspace{1cm}\left\|c_4^\text{new}-c_4^\text{old}\right\|_{\infty}\sim\mathcal{O}\left(10^{-13}\right), 
\end{align}
Only the norm for $F_{n}$ is approximately $10^{3}$ higher than the others, implying that equation for $\varv_{F}$ may have an internal conflict. The form of equation has following mathematical structure
\begin{align}
&\left(\frac{1+x}{2}\right)^{a+1}\frac{\text{d}\varv_{F}(x)}{\text{d}x}\mathcal{\eta}(x;\varv_{G},\varv_{K})+\left(\frac{1+x}{2}\right)^{a}\mathcal{\mu}(x;\varv_{G},\varv_{K})+c_{1}e^{-\varv_{F}(x)}(\varv_{J}+1)=0.\label{Eq.1ODE}\\
&\left(\frac{1+x}{2}\right)^{a+1}\frac{\text{d}\varv_{F}(x\to-1)}{\text{d}x}+\left(\frac{1+x}{2}\right)^{a}\mathcal{\mu}(x;\varv_{G},\varv_{K})+c_{1}e^{-\varv_{F}(x)}(\varv_{J}(-1)+1)=0.
\end{align}
In equation \eqref{Eq.1ODE} as $x\to1$ the second term takes the value $a$ while the third term takes the value $c_{1}$ $(\sim10^{-3})$. Considering the fact the eigenvalues $c_{1}$ and $c^{*}_{4}$ is imperative to $F_\text{BC}$, the effective machine precision may be considered approximately  $10^{3}$ greater than the that of MATLAB. For example, In the factor $(1+\varv_{J})\propto\left(\frac{1+x}{2}\right)^{a}$, meaning the last term can be considered numerically zero at equation level if the value of $\left(\frac{1+x}{2}\right)$ reaches a new machine precision $\text{eps}/c_{1})\approx 2.5\times10^{-13}$. This could explain the relation in equation \eqref{Eq.1ODE} though, the actual accuracy would rely on the minimum of the value $\varv_{I}(x\to1)$;
\begin{align}
\min{\varv_{I}(x\to1)}\sim\mathcal{O}(10^{-12})
\end{align}
which well explains that all the Chebyshev coefficients stalls at $\mathcal{O}(10^{-12})$ together with $\varv_{I}(x\to1)$ can reach order of $10^{-12}$. This relation determines the practical end point $x_\text{p.e}$ near $x=-1$ which is  $ x_\text{p.e}\approx-0.93$; one can not meaningfully solve the equation outside the domain $(x_\text{p.e})<x<1$ since the double precision would be not enough. Also the accuracy $1\times10^{-12}$ would constraint the first term in equation \eqref{Eq.1ODE}. As explained in section \ref{sec:ss_soln_entire}, the variable $\varv_{F}$ is approximately proportional to $\left(\frac{1+x}{2}\right)^{a}$; the $\varv_{F}(x)$ approach $\ln[c^{*}_{4}]$ at $x<x_\text{const}$ where $x_\text{const}\approx-0.63$ is obtained by solving $\left(\frac{1+x}{2}\right)^{2a}=1\times10^{-13}$ for $x$. The results obtained in section \ref{sec:ss_soln_entire} reflects the range of domain; the constancy of $\varv_{I}-\varv_{I}$ is covered on the domain $x_\text{p.e}<x<x_\text{const}$ and the function is no longer constant at $x<x_\text{p.e}$. 


From the relationship in accuracies among $\beta$, $c_{1}$ and $c^{*}_{4}$ and the interpretation, one may guess the cause of difficulty in Newton iteration procedure. First, there exist a gap of $\sim1\times10^{3}$ in accuracy between $c^{*}_{4}$ and $\varv_{K}(x=1)$. The gap would originate from the fact that the constancy is valid at least at $x_\text{const}\approx-0.63$ which results in an internal gap in the variable $F(E)/c1\left(\propto\left(\frac{1+x}{2}\right)^{a}\right)/c1$ by a factor of $\left(\frac{1+x_\text{const}}{2}\right)^{a}\approx1\times10^{3}$. This means one needs approximately an accuracy of $10^{-5}$ to solve the equation for $c^{*}_{4}$ with one significant figure.  
 
 

==> Section7_Thermo.tex <==
\section{Thermodynamic aspects of the ss-OAFP model}\label{sec:Thermo}

\hspace{0.6cm} Infinite isotropic models (the isothermal- and polytropic spheres and ss-OAFP models) are not suitable for practical applications to compare them to observed data. Rather, since they somehow originate from statistical principles, they have been employed to deepening one's understanding of self-gravitating systems. In the present section, basic (analogue of) thermodynamic aspects of the ss-OAFP model is discussed; those of the isothermal- and polytropic- spheres and King models have been discussed while the ss-OAFP model has not been discussed yet. Section \ref{sec:Diff_models} explains isotropic models typically used for this matter.  Section \ref{sec:Thermo_Quan_ss_FP} shows the thermodynamic- and hydrodynamic- quantities of the self-similar model. In Section \ref{sec:Reg_C-curve} the quantities are regularized and negative specific heat at constant volume is shown by constructing an analogue of caloric curve. Lastly, Section \ref{sec:Virial} discusses based on the Virial ratio and Virial, the instability of the ss-OAFP model enclosed by an adiabatic wall.


\subsection{Isotropic self-gravitating models}\label{sec:Diff_models}

\hspace{0.6cm}The isotropic models to establish equilibrium statistical mechanics of self-gravitating (gaseous) system may be listed based on what temperature is considered as follows;
\begin{align}
&\text{\emph{Isothermal sphere} \citep{Antonov_1985,Lynden_Bell_1968}},\nonumber\\ 
&\text{\emph{\,    }} \hspace{3.0cm}  \text{Thermodynamic temperature (Boltzmann entropy)}\nonumber\\
&\text{\emph{Energy-truncated models} \citep{Katz_1980,Katz_1983}},\nonumber\\
 &\text{(e.g. King, Woolley, and Wilson  models)} \nonumber\\
&\text{\emph{\,    }} \hspace{3.0cm} \text{Thermodynamic temperature  (Phenomelogical entropies)}\nonumber\\
&\text{\emph{Polytropic sphere}} \hspace{0.5cm} \text{Local thermodynamic temperature }  \nonumber\\
&\text{\emph{Stellar Polytrope} \citep{Taruya_2002,Chavanis_2002_poly}} \nonumber\\
&\text{\emph{\,    }} \hspace{3.0cm} \text{Polytropic temperature or constant (Tsallis's entropy)}  \nonumber\\
&\text{\emph{ss-OAFP models}} \hspace{0.5cm} \text{Out of thermodynamic equilibrium}  \nonumber
\end{align}
The ss-OAFP model perhaps can have three different (non-)equilibrium and QSS states. In the core the stars could behave like an isothermal sphere due to frequent two-body relaxation events. The inner halo would be a receiver of heat- and particle- fluxes due to the escaping stars from the core, resulting in a nonequilibrium stationary state. In the outer halo, in self-similar analysis\footnote{More realistically in two dimensional (anisotropic) case, escapers and escaping stars with high eccentricity under the influence of tidal effects form the outer halo.} the extension of inner halo without or with very little particle- and energy- fluxes would behave like a collisionless system forming a power-law profile at a state of Tsallis equilibrium.

Yet, the ss-OAFP system could need some extra assumptions compared to the other models. For example, the system assume to be valid only in an time-averaged sense due to the discreteness. Hence, to consider the system a thermodynamic system, the system is assumed to be an 'exotic' self-gravitating gas at a stationary non-equilibrium state, composed of $N_\text{T}(>>10^{6}>>1)$ particles whose DF and m.f. potential follow the solution of the ss-OAFP model at a certain epoch. The meaning of 'exotic' is here that the gas has intrinsically \emph{negative} specific heat as its normal state (at least in the core of the system) as will be explained in the following sections. Also, following the classical discussion \citep{Antonov_1985,Lynden_Bell_1968} for simplicity, consider the ss-OAFP model of $N_\text{T}$ can be enclosed by an adiabatic spherical wall of radius $R(\Phi)$ that elastically reflects star on the inner surface. The present section employs the reference solutions $F_\text{o}(E)$ and $\Phi(R_\text{o})$.
 
\subsection{Thermodynamic quantities of self-similar evolution model}\label{sec:Thermo_Quan_ss_FP}

\hspace{0.6cm} Sections \ref{sec:LTQ} and \ref{sec:GTQ} show the local- and global- thermodynamic quantities to see the characteristics of the ss-OAFP model. 

\subsubsection{Local Thermodynamic quantities}\label{sec:LTQ}

\hspace{0.6cm} Since the DF for the ss-OAFP model is not a Maxwellian DF, (possibly not even local one anywhere the system), hence discussion of local thermodynamic- or hydrodynamic- quantities is imperative to capture the nature of the model. In addition to density $D(\Phi)$, the velocity dispersion, pressure and heat- and particle- fluxes may be defined in terms of moments of DF of stars 
\begin{subequations}
\begin{align}
&\varv^{2}(r,t)=\frac{1}{\rho(r,t)(\phi)}\int^{0}_{\phi(r,t)}(2\epsilon-2\phi(r,t))^{3/2}f(\epsilon,t)\text{d}\epsilon,\\
&p(r,t)=\frac{\varv^{2}(r,t)\rho(r,t)}{3},\\
&\mathcal{f}^\text{h}(r,t)=-\mathcal{k}\frac{\partial \varv^{2}}{\partial{r}},\\
&\mathcal{f}^\text{p}(r,t)=-\mathcal{D}\frac{\partial \rho(r,t)}{\partial{r}},
\end{align}
\end{subequations}
where $\mathcal{k}$ is the thermal conductivity and $\mathcal{D}$ the diffusivity. Since the value of $\mathcal{k}$ (and $\mathcal{D}$) depends on the definition of relaxation time concerned \citep{Lynden_Bell_1980,Louis_1991} it is convenient to regularize the heat- and particle- fluxes by the constants in the coefficients in self-similar analysis (by $3GmC_\text{k} \ln[N_\text{T}]$ for the conductivity and $\sqrt{2 C_\text{D}\ln[N_\text{T}]/3}$ for the diffusivity\footnote{For the conductivity the expression followed \citep{Lynden_Bell_1980}. In a similar way, the diffusivity is calculated as follows
\begin{align}
\mathcal{D}=\frac{1}{3}l\sqrt{\varv^{2}}\approx\frac{1}{3k_{J}^{2}}\frac{C_\text{D}}{T_{R}}=\frac{1}{3}\frac{\varv^{2}(r,t)}{4\pi G \rho(\phi(r,t))}\frac{8\pi Gm C_\text{D}\rho(\phi,t)\ln[N_\text{T}]}{[\varv^{2}(r,t)]^{3/2}}=\frac{2C_\text{D}\ln[N_\text{T}]}{3\sqrt{\varv^{2}(r,t)}},
\end{align}
where $l$ is the mean free path, $k_\text{J}$ is the inverse of Jeans length and $T_{R}$ is the relaxation time from \citep{Spitzer_1988}.}, where $C_\text{k}$ and $C_\text{D}$ are dimensionless constants of approximately unity.). Employing the self-similar variables of Section \ref{sec:math_formul} and introducing new self-similar variables
\begin{subequations}
\begin{align}
&\varv^{2}(r,t)=V^{2}_\text{(dis)}(R)\varv^{2}_\text{t}(t)\equiv 2V_\text{(dis)}^{2}(R)\epsilon_\text{t}(t),\\
&p(r,t)=P(R)p_\text{t}(t),\\
&\frac{\mathcal{f}^\text{h}(r,t)}{3GmC_\text{k} \ln[N_\text{T}]}\equiv\mathcal{F}^\text{h}(R)\mathcal{f}^\text{h}_\text{t}(t),\\
&\frac{\mathcal{f}^\text{p}(r,t)}{2C_\text{D} \ln[N_\text{T}]/3}\equiv\mathcal{F}^\text{p}(R)\mathcal{f}^\text{p}_\text{t}(t),
\end{align}
\end{subequations}
where $S(\Phi)=-2S(x)$ due to the definition, one can obtain the quantities in self-similar form
\begin{subequations}
\begin{align}
&V_\text{(dis)}^{2}(R)=2\frac{U_{3/2}(\Phi)}{U_{1/2}(\Phi)},\\
&P(R)=\frac{2}{3}U_{3/2}(\Phi),\\
&\mathcal{F}^\text{h}(R)=-\frac{U_{1/2}(\Phi)}{S(\Phi)\sqrt{V_\text{(dis)}^{2}(\Phi)}}\left(\frac{U_{3/2}(\Phi)U_{-1/2}(\Phi)}{[U_{1/2}(\Phi)]^{2}}-3\right),\\
&\mathcal{F}^\text{p}(R)=-\frac{1}{\sqrt{V_\text{(dis)}^{2}(\Phi)}}\frac{U_{-1/2}(\Phi)}{S(\Phi)},
\end{align}
\end{subequations}
where the integral $U_{n}(\Phi)$ was introduced as
\begin{align}
U_{n}(\Phi)=\int^{0}_{\Phi}F(E)(E-\Phi)^{n}\text{d}E.
\end{align}
where $n$ is a real number; for example, if $n=1/2$  then $U_{n}(\Phi)=D(\Phi)$. 

The velocity dispersion and heat flux are depicted in Figure \ref{Fig.R_Phi_Vdis_HeatF_DensF_Tr}(a) and have a similar characteristics reported in \citep{Lynden_Bell_1980} for self-similar gaseous model. The constancy of velocity dispersion is further extended in radius compared to the m.f. potential profile. The heat flux reaches its maximum at $R=4.31$; the radius is relatively close to $R=8.99$ at which the gravaothermal instability occurs for the isothermal sphere in canonical ensemble \citep{Lynden_Bell_1968}.  The particle flux reaches its maximum at slightly smaller radius, $R=3.11$. As the half-mass relaxation time increases with radius, the both fluxes rapidly decreases; the particle flux decays slightly slow compared to the heat one.

As discussed in \citep{Cohn_1980}, one may see the signature of gravothermal instability based on polytropic index $m\equiv\beta_\text{o}+3/2$ in the core of cluster.  Figure  \ref{Fig.R_AdiaIndex_m_ss} shows the adiabatic index $\Gamma (\equiv1+1/m)$ and polytropic index $m$ against dimensionless radius; the adiabatic index was obtained by calculating the logarithmic derivative $\text{d}\ln[P(R)]/\text{d}\ln[D(R)]$. The result shows a distinctive nature in the structure of core, inner-halo and outer-halo. In the outer halo, the polytropic index asymptotically reaches $m=9.67837115... (\Gamma\approx1.10)$  for large $R$. \footnote{The value of $m$ holds the relative error $6.3\times10^{-10}\%$  from the expected value $\beta_\text{o}+3/2$.} For small radii or in the core and inner halo, one can find two distinctive characteristics. (i) the index takes its minimum value $m=8.52$ $(\Gamma=1.117)$ at $R=157$; (ii) the index decreases with decreasing radius at small radii and at the very center of the core the polytropic index reaches 
$177$ $ (\Gamma=1.00564)$. Higher polytropic  indeces (or adiabatic indeces close to unity) for the core imply the core behaves like an isothermal sphere. 

Making use of the given adiabatic indeces, one can find the asymptotic form for the equation of local state numerically (Figure \ref{Fig.R_LocEqnState}). At the core, as expected, the core may be described by an ideal gas with the thermodynamic temperature $1/\beta^\text{(con)}$ while the outer halo follows a polytrope of $m=\beta_\text{o}+3/2$ and has a temperature approximately half of $1/\beta^\text{(con)}$ if the polytropic constant $K$ (in $p(r,t)=K\rho(r,t)^{\Gamma}$) is considered the constant temperature of the polytrope; 
\begin{align}
&P= \frac{1.0}{\chi_\text{esc}}D, \hspace{1cm} (R\approx 0)\\
&P= \frac{0.5}{\chi_\text{esc}}D^{\Gamma}. \hspace{1cm} (R\to \infty)
\end{align} 
where it is to be noted in the present self-similar analysis the inverse temperature $\beta^\text{(con)}$  must be replaced by $\chi_\text{esc}$.
\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{loglogaxis}[width=8cm,height=8cm,
	grid=major,xlabel=\Large{$R$},xmin=1e-1,xmax=1e5,ymin=1e-2,ymax=1.2e0,legend pos=south west]
	\addplot [color = red ,mark=no,thick,densely dashed ] table[x index=0, y index=1]{R_Phi_Vdis_HeatF_DensF_InvTr.txt};
	\addlegendentry{\large{$\mid\Phi\mid$}} 
	\addplot [color = blue ,mark=no,thick,solid ] table[x index=0, y index=1]{R_LocT_KinT.txt};
	\addlegendentry{\large{$V\text{(dis)}^{2}$}}
      \node[above,black] at (4e4,0.7) {(a) };
	\end{loglogaxis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{loglogaxis}[width=8cm,height=8cm,
	grid=major,xlabel=\Large{$R$},xmin=1e-1,xmax=1e8,ymin=1e-24,ymax=1.1e1,legend pos=south west]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=3]{R_Phi_Vdis_HeatF_DensF_InvTr.txt};
	\addlegendentry{\Large{$\mathcal{F}^\text{h}$}} 
	\addplot [color = orange ,mark=no,thick,densely dashed ] table[x index=0, y index=4]{R_Phi_Vdis_HeatF_DensF_InvTr.txt};
	\addlegendentry{\Large{$\mathcal{F}^\text{p}$}} 
      \addplot [color = blue ,mark=no,thick,densely dotted] table[x index=0, y index=5]{R_Phi_Vdis_HeatF_DensF_InvTr.txt};
	\addlegendentry{\Large{$1/\tilde{T}_\text{R}$}} 
      \node[above,black] at (4e7,0.1) {(b) };
	\end{loglogaxis}
	\end{tikzpicture}
	\caption{Dimensionless m.f. potential $\Phi$ and velocity dispersion $V\text{(dis)}^{2}$ (left) and dimensionless heat flux $\mathcal{F}^\text{h}$ and particle flux $\mathcal{F}^\text{p}$(right). The inverse of regularized half-mass relaxation time $\tilde{T}_\text{R}$ $\left(=D(\phi,t)/[\varv^{2}(r,t)^{3/2}\right)$ is also shown for comparison.}
	\label{Fig.R_Phi_Vdis_HeatF_DensF_Tr}
\end{figure}  

\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{semilogxaxis}[width=12cm,height=6cm,
	grid=major,xlabel=\Large{$R$},ylabel=\Large{$\Gamma$},xmin=1e-1,xmax=1e17,ymin=9.5e-1,ymax=1.2e0,legend pos=south east]
	\addplot [color = blue ,mark=no,thick,solid] table[x index=0, y index=1]{R_AdiaIndex.txt};
	\end{semilogxaxis}
      \end{tikzpicture}
      \begin{tikzpicture}
	\begin{semilogxaxis}[width=12cm,height=6cm,
	grid=major,xlabel=\Large{$R$},ylabel=\Large{$m$},xmin=1e-1,xmax=1e17,ymin=0,ymax=180,legend pos=south east]
      \addplot [color = blue ,mark=no,thick,solid] table[x index=0, y index=1]{R_m_ss.txt};
	\end{semilogxaxis}
      \end{tikzpicture}
	\caption{Adiabatic index $\Gamma$ and polytropic index $m$ of the ss-OAFP model.}
	\label{Fig.R_AdiaIndex_m_ss}
\end{figure}  

\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{semilogxaxis}[width=11cm,height=7cm,
	grid=major,xlabel=\Large{$R$},ylabel=\Large{$P\chi_\text{esc}/D$},xmin=1e-1,xmax=1e18,ymin=0.1,ymax=1.2e0,legend pos=north east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=1]{R_LocEqnState.txt};
	\end{semilogxaxis}
	\end{tikzpicture}\caption{Local equation of state with constant thermodynamic temperature $\beta^\text{(con)}$.}
	\label{Fig.R_LocEqnState}
\end{figure}  


\subsubsection{Thermodynamic quantities}\label{sec:GTQ}

\hspace{0.6cm} The discussion of (global) thermodynamic quantities is a marginal importance due to the difficulty in conceptualizing temperature, entropy and the thermodynamic zeroth law. It will, however, provide a good insight for understanding the nature of macroscopic structure as comparison to the result of Section \ref{sec:LTQ}. The total- mass, kinetic energy and potential energy of stars that are confined by adiabatic wall at radius $R_\text{M}$ read
\begin{subequations}
	\begin{align}
	&M(R_\text{M},t)=\iint m f(\epsilon,t)\text{d}^{3}\varv\text{d}^{3}r,\\
	&\text{KE}(R_\text{M},t)=\iint m\frac{\varv^{2}}{2}f(\epsilon,t)\text{d}^{3}\varv\text{d}^{3}r,\\
	&\text{PE}(R_\text{M},t)=\iint m\phi(r,t)f(\epsilon,t)\text{d}^{3}\varv\text{d}^{3}r,\\
	&E_\text{tot}(R_\text{M},t)=\text{KE}+\text{PE}.
	\end{align}
\end{subequations}
The self-similar forms are as follows
\begin{subequations}
	\begin{align}
	&M(\Phi_\text{M})\equiv\frac{M(r,t)}{M_\text{t}(t)}=-\int^{\Phi_\text{M}}_{-1}DR^{2}S\text{d}\Phi,\\
	&\text{KE}(\Phi_\text{M})\equiv\frac{\text{KE}(r,t)}{\text{PE}_\text{t}(t)}=-\int^{\Phi_\text{M}}_{-1}U_{3/2}R^{2}S\text{d}\Phi,\\
	&\text{PE}(\Phi_\text{M})\equiv\frac{\text{PE}(r,t)}{\text{PE}_\text{t}(t)}=\frac{1}{2}\int^{\Phi_\text{M}}_{-1}\Phi DR^{2}S\text{d}\Phi,\\
	&E_\text{tot}(\Phi_\text{M})\equiv\frac{E_\text{tot}(r,t)}{PE_\text{t}(t)},
	\end{align}
\end{subequations}
where $\Phi_{M}$ is the potential at the wall radius $R_{M}$ and the corresponding time-dependent variables have the following relation
\begin{subequations}
	\begin{align}
	&M_\text{t}(t)= (4\pi)^{2}\sqrt{2} m f_\text{t}(t)[E_\text{t}(t)]^{3/2}[r_\text{t}(t)]^{3},\\
	&\text{PE}_\text{t}(t)=\frac{\text{KE}_\text{t}(t)}{2}=\frac{1}{2}M_\text{t}(t)E_\text{t}(t).
	\end{align}
\end{subequations}

Since the thermodynamic temperature can not be defined, one may heuristically introduce the kinetic temperature $T^\text{(kin)}$ and local temperature $T^\text{(loc)}$
\begin{subequations}
\begin{align}
&T^\text{(kin)}(\Phi_\text{M})\equiv\frac{2\text{PE}}{3M},\\
&T^\text{(loc)}(R_\text{M})\equiv\frac{V_\text{(dis)}^{2}}{3}.
\end{align}
\end{subequations}
The local- and kinetic- temperatures are depicted in Figure \ref{Fig.R_LocT_KinT}. At the center of the system the temperatures holds approximately a constant profile.\footnote{Of course exactly speaking, the temperatures gradually decreases with radius and the maximum temperatures are lowered by 1 $\%$ approximately at $R\approx2.1$ for local temperature and $R\approx2.7 $ for kinetic one.} Hence, if one focuses on the specific heat in the core, inverse temperature of Maxwellian DF in standard context of statistical mechanics can be defined as 
\begin{align}
\beta^\text{(con)}=\frac{\chi_\text{esc}}{\epsilon_{t}(t)},
\end{align}
where $\chi_\text{esc}$ was introduced to change the boundary condition for Poisson equation from $\Phi(R)=-1$ to $\Phi(R)=-\chi_\text{esc}$ so that one can directly compare the present result to the isothermal sphere. This provides an approximate relationship at the center of the system
\begin{subequations}
\begin{align}
&T^\text{(loc)}R_\text{M}r_\text{t}(t)\approx T^\text{(kin)}R_\text{M}r_\text{t}(t)\approx \frac{1}{k_\text{B}\beta^\text{(con)}},\\
&T^\text{(loc)}(\Phi_{M})\approx T^\text{(kin)}(\Phi_{M})\approx \chi_\text{esc},
\end{align}
\end{subequations}
where $k_\text{B}$ is the Boltzmann constant. 
 

   
\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{loglogaxis}[width=8cm,height=8cm,
	grid=major,xlabel=\Large{$R$},xmin=1e-1,xmax=1e15,ymin=1e-4,ymax=1.2e0,legend pos=north east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=1]{R_LocT_KinT.txt};
	\addlegendentry{\large{$ T^\text{(loc)}$}}
	\addplot [color = blue ,mark=no,thick,densely dashed ] table[x index=0, y index=2]{R_LocT_KinT.txt};
	\addlegendentry{\large{$ T^\text{(kin)}$}}
	\end{loglogaxis}
	\end{tikzpicture}\caption{Local temperature and kinetic temperature.}
	\label{Fig.R_LocT_KinT}
\end{figure}  




\subsection{Regularization of thermodynamic quantities and negative specific heat}\label{sec:Reg_C-curve}

\hspace{0.6cm}The present section focuses especially on the core of the ss-OAFP model to see the negative specific heat. In Section \ref{sec:reg_thermo} the total energy and temperature are regularized and in Section \ref{sec:C-curve} the caloric curve is shown to characterize the negative specific heat.

\subsubsection{Regularized thermodynamics quantities}\label{sec:reg_thermo}

\hspace{0.6cm}One's expectation for establishing a thermodynamic system is that there exist certain thermodynamic limits as standard limit says $N_\text{T}/V\to $ const. if $N_\text{T}\to\infty$ and $V\to\infty$ for short-range interacting system. Also, since the mass, energy and size of the ss-OAFP model are infinite, one needs a proper thermodynamic limit to regularize thermodynamic quantities with $R_\text{M}$. For total energy, the following normalized energy has been employed for isothermal sphere \citep{Antonov_1985,Lynden_Bell_1968} based on Boltzmann entropy and polytrope \citep{Taruya_2002,Chavanis_2002_poly} based on Tsallis entropy
\begin{align}
\Lambda=\frac{rE_\text{tot}(r,t)}{GM^{2}(r,t)}=\frac{R_\text{M}E_\text{tot}(\Phi_{M})}{\left[M(\Phi_{M})\right]^{2}}.
\end{align}\label{Eq.norm_E}
Figure \ref{Fig.R_Lambda_Eta} shows the normalized total energy; the energy is negative at all radii, meaning that the system is dominated by the potential energy as expected for collapsed phase. The normalized energy reaches order of unity in the following limit with $N_\text{T}$ (sometimes called the \emph{dilute} limit that more formally correspond to one of Boltzmann-Knudsen limits in standard gaseous kinetic theory)
\begin{subequations}
	\begin{align}
	&R_\text{M}\propto N_\text{T},\\
	&M(\Phi_{M})\propto N_\text{T},\\
	&E_\text{tot}(\Phi_{M})\sim \text{KE}(\Phi_{M})\sim \text{PE}(\Phi_{M})\propto N_\text{T},\\
	&1/\beta^\text{(con)}\propto 1,
	\end{align}
\end{subequations}
where one should recall the thermodynamic limit just determines the relation among the magnitudes of quantities; the important point is that some reasonable dimensionless parameter exist.\footnote{Well-acknowledged density (cluster) expansion in thermodynamic limit does not mean a density $n$ itself is the expansion parameter, rather the corresponding (dimensionless) occupation number $\frac{4}{3}na^3$, where $a$ is the characteristic size of particles, is the actual parameter.} In a similar way, one can normalize the reciprocal of the kinetic-, local- and thermodynamic- temperatures in normalized form as follows
\begin{subequations}
	\begin{align}
	&\eta^\text{(kin)}=\frac{GM(R_\text{M}r_\text{t}(t),t)}{k_\text{B}T^\text{(kin)}(R_\text{M}r_\text{t}(t)})=\frac{M}{T^\text{(kin)}R_\text{M}},\\
	&\eta^\text{(loc)}=\frac{GM(R_\text{M}r_\text{t}(t),t)}{k_\text{B}T^\text{(loc)}(R_\text{M}r_\text{t}(t))}=\frac{M}{T^\text{(loc)}R_\text{M}},\\
	&\eta^\text{(con)}=\frac{\beta^\text{(con)} R_\text{M}r_\text{t}(t)}{GM(R_\text{M}r_\text{t}(t))^2}=-\frac{S(\Phi_\text{M})}{R_\text{M}}.
	\end{align} \label{Eq.norm_T}
\end{subequations}
The normalized temperatures are shown in Figure \ref{Fig.R_nTkin_nTloc_nTcon}. All the temperatures monotonically decreases with radii until they reach the minimum values. Only $\eta$ does diverge with $R$ which implies that the inverse temperature $\beta^\text{(con)}$ is not correctly regularized; it is better to be regularized as if it is a polytropic sphere of $m=\beta_\text{o}+3/2$



\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{loglogaxis}[width=8cm,height=8cm,
	grid=major,xlabel=\Large{$R_\text{M}$},ylabel=\Large{$-\Lambda$},xmin=1e-1,xmax=1e20,ymin=1e0,ymax=1e2,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=1]{R_NegLambda_InvLambda_Eta_InvEta.txt};
	\end{loglogaxis}
     \end{tikzpicture}
\caption{Dimensionless normalized total energy.}
	\label{Fig.R_Lambda_Eta}
\end{figure}  



\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{loglogaxis}[width=10cm,height=6cm,
	grid=major,ylabel=\Large{$\eta^\text{(kin)}$},xmin=1e-1,xmax=1e20,ymin=1e-1,ymax=1e3,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=1]{R_nTkin_nTloc_nTcon.txt};
	\end{loglogaxis}
	\end{tikzpicture}
     \begin{tikzpicture}
	\begin{loglogaxis}[width=10cm,height=6cm,
	grid=major,ylabel=\Large{$\eta^\text{(loc)}$},xmin=1e-1,xmax=1e20,ymin=1e-1,ymax=1e3,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=2]{R_nTkin_nTloc_nTcon.txt};
	\end{loglogaxis}
	\end{tikzpicture}
    \begin{tikzpicture}
	\begin{loglogaxis}[width=10cm,height=6cm,
	grid=major,xlabel=\Large{$R_\text{M}$},ylabel=\Large{$\eta^\text{(con)}$},xmin=1e-1,xmax=1e20,ymin=1e-1,ymax=1e4,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=3]{R_nTkin_nTloc_nTcon.txt};
	\end{loglogaxis}
	\end{tikzpicture}
\caption{Dimensionless normalized temperatures.}
	\label{Fig.R_nTkin_nTloc_nTcon}
\end{figure}  

\subsubsection{Caloric curve}\label{sec:C-curve}

\hspace{0.6cm}Based on the dimensionless energy \eqref{Eq.norm_E} and temperatures \eqref{Eq.norm_T}, one may construct a caloric curve at constant volume (Figure \ref{Fog.R_InvLamb_INVnTkin_INVnTloc_INVnTcon}). Based on Legendre transform one still can relate the graph to the  specific heat $C_\text{V}$; for example the kinetic temperature results in the following relation 
\begin{align}
\left(\frac{\partial \frac{1}{\Lambda}}{\partial \eta^\text{(kin)}}\right)_{R,M}=\left(\frac{\partial \frac{1}{\Lambda}}{\partial \eta^\text{(kin)}}\right)_{V,N_{tot}}=\frac{C_\text{V}\left[T^\text{(kin)}\right]^{2}}{ME_\text{tot}^{2}}.
\end{align}
The advantage of the caloric curve approach is to provide a simple topological understanding for the stability of systems in statistical (e.g. microcanonical- and canonical-) ensembles without solving the eigenvalue problem \citep{Katz_1978,Katz_1979,Katz_1980}. Of course the present interest is only the \emph{analogue} of the ensembles since the ss-OAFP can not be at a state of thermodynamic equilibrium. In Figure \ref{Fog.R_InvLamb_INVnTkin_INVnTloc_INVnTcon}, all the caloric curves show negative specific heat at small radii while they show different characteristics at larger radii after passing through their turning points. The turning points of the caloric curves (Table \ref{table:C-curve_Tuning}) occurs very close to each other in radius ($R\approx18\sim 24$ for $C_\text{V}\to\infty$ and $R\approx25$ for $C_\text{V}=0$ ). This might be consistent with characteristics of gravothermal instability. The negative heat capacity of the core would originate from the independence of the core from the halo (other than releasing particles and heat to the inner halo). This implies that regardless of kinds of walls (adiabatic, thermal or rubber) and ensemble (microcanonical, canonical, isobaric ), the singular behaviors in the specific heat (instability) could occur very close to each other in radius \emph{outside} the radius at which the heat flux reaches its maximum at $R=4.31$. 


\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{axis}[width=7cm,height=8cm,
	grid=major,xlabel=\Large{$\eta^\text{(kin)}$},ylabel=\Large{$1/\Lambda$},xmin=0,xmax=3,ymin=-0.3,ymax=0,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=2, y index=1]{R_InvLamb_INVnTkin_INVnTloc_INVnTcon.txt};
	\end{axis}
	\end{tikzpicture}
    \begin{tikzpicture}
	\begin{axis}[width=7cm,height=8cm,
	grid=major,xlabel=\Large{$\eta^\text{(con)}$},xmin=0,xmax=3,ymin=-0.3,ymax=0,legend pos=south east]
	\addplot [color = orange ,mark=no,thick,solid ] table[x index=4, y index=1]{R_InvLamb_INVnTkin_INVnTloc_INVnTcon.txt};
	\end{axis}
	\end{tikzpicture}
 \begin{tikzpicture}
	\begin{axis}[width=7cm,height=8cm,
	grid=major,xlabel=\large{$\eta^\text{(loc)}$},ylabel=\Large{$1/\Lambda$},xmin=0,xmax=3,ymin=-0.3,ymax=0,legend pos=south east]
	\addplot [color =blue ,mark=no,thick,solid ] table[x index=3, y index=1]{R_InvLamb_INVnTkin_INVnTloc_INVnTcon.txt};
	\end{axis}
	\end{tikzpicture}
 \begin{tikzpicture}
	\begin{axis}[width=7cm,height=8cm,
	grid=major,xlabel=\large{$\eta^\text{(loc)}$},xmin=2.4,xmax=2.8,ymin=-0.29,ymax=-0.22,legend pos=south east]
	\addplot [color = blue ,mark=no,thick,solid ] table[x index=3, y index=1]{R_InvLamb_INVnTkin_INVnTloc_INVnTcon.txt};
	\end{axis}
	\end{tikzpicture}
\caption{Caloric curves for the normalized- temperatures ($\eta^\text{(kin)}$,  $\eta^\text{(loc)}$ and $\eta^\text{(con)}$) and total energy ($\Lambda$). For graphing purpose, reciprocal of $\Lambda$ is shown for the ordinates; the tangent to the curve represents the kinetic specific heat.}
	\label{Fog.R_InvLamb_INVnTkin_INVnTloc_INVnTcon}
\end{figure}  

\begin{table*}\centering
	\ra{1.3}
	\begin{tabular}{@{}l|cccc|cccc@{}}\toprule
		               &$C_\text{V}\to\infty$ &    &&         & $C_\text{V}=0$ &  & &\\ 
		\midrule
		             & $\eta$ & $\Lambda$&$R_\text{M}$ & $D(0)/D(R_\text{M})$ &$\eta$& $\Lambda$ &$R_\text{M}$ & $D(0)/D(R_\text{M})$  \\ 
		\midrule
		Kinetic & 2.580  &-3.599  &  19.2   &  36.6  &2.540&          &    &\\
	    Local   & 2.712  &-3.549  &  24.1   &  65.8  &2.711& -3.548&25.4&74.85\\
		Thermodynamic & 2.492  &-3.633  &  17.9   &  30.3  &2.418&          &    &\\
		\midrule
		IS      &        &-0.335  &  34.4   &  709   &2.52&          &8.99   &32.1\\
		\bottomrule
	\end{tabular}\\
	\caption{First turning points of caloric curves at small radii. IS is the corresponding values for the isothermal sphere.}
	\label{table:C-curve_Tuning}
\end{table*}


The negative specific heat in the core was an expected property for the ss-OAFP model. Yet, comparing the results between the local- and global- thermodynamic quantities, it is not clear at first place to see the origin of the negative specific heat of the model since the heat- and particle- fluxes, polytropic index and equation of local state show the characteristics of the isothermal sphere in the core. The difference from the isothermal sphere originates from the total potential energy being \emph{very} greater than total kinetic energy. Figure \ref{Fig.R_PeKeRatio_regVirial}(a) shows the Virial ratio; the ratio is smaller than unity at all radii implying that the potential energy dominates the total energy or in `collapsed' phase, which occurs to isothermal sphere, polytropes ($m>5$) and King model with large $R_\text{M}$. More specifically, the deep potential well, of course, originates from the \emph{large} scaled escape energy $(\approx13.88)$ of DF in the present work.  To see if this statement is correct, one can reduce the total energy to the following form
\begin{align}
E_\text{tot}=\int^{R_\text{M}}_{0}\text{d}R\int^{0}_{\Phi}\text{d}E/,\Omega_\text{tot}(E,\Phi)R^{2}(E)(E-\Phi)^{3/2},
\end{align}
where the kernel $\Omega_\text{tot}(E,\Phi)$ is defined as follows
\begin{align}
\Omega_\text{tot}(E,\Phi)=F(E)-\frac{\Phi}{3}\frac{\text{d}F}{\text{d}E}.\label{Eq.intgerand kernal}
\end{align}
Equation \eqref{Eq.intgerand kernal} presents a quite-easy analytical method for the sign of specific heat in the core. For example, if one assumes DF behaves like the isothermal sphere with scaled escape energy $\chi_\text{esc}$; the dimensionless DF is $F(E)=\exp[\chi_\text{esc}E]$;
\begin{align}
\Omega_\text{tot}(E,\Phi)=e^{\chi_\text{esc}E}\left(1-\frac{\chi_\text{esc}}{3}\Phi\right).\label{Eq.Omega}
\end{align}
The threshold of the potential energy is greater than kinetic energy is given as 
\begin{align}
\Phi^\text{(th)}=-\frac{3}{\chi_\text{esc}}.\label{Eq_crit_neg_PEKE}
\end{align}
In case of the isothemal gas sphere ($\chi_\text{esc}=1$), $\Omega_\text{tot}(E,\Phi)$ is necessary positive at $R<3\sqrt{2}$ if one uses  $\Phi(R\approx0)=-R^{2}/6$.\footnote{Or $R<7.46$ if one employs a numerical result \citep{Ito_2018} for the Lane-Emden equation for isothermal sphere.} Since the regularized temperature is defined only from the Poisson equation as $-R/S$ which is  monotonically increasing with R; the positive specific heat is always secured in the core for isothermal sphere. (Considering that the negative specific heat occurs at radii larger than $R=8.99$, this simple discussion is consistent). On one hand, the ss-OAFP model may be modeled by the same kernel \eqref{Eq.Omega} with $\chi_\text{esc}=13.88$. This is since the reference DF $F_\text{o}(E)$ well fits the exponential of $\chi_\text{esc}E$ on interval $-1<E<-0.3$ and $\exp[-\chi_\text{esc}0.3]$ contributes with small amount of value  $\sim 6\times10^{-5}$ at the end ($E\approx-0.3$). In limit of $R\to0$, one can employ the same logic above. The temperature in the core even for ss-OAFP model is relatively constant and the characteristics are well shown in Figure \ref{Fig.R_nTkin_nTloc_nTcon} with decreasing normalized temperatures at small radii.  Hence, the ss-OAFP model has a negative total energy at small radii less than $R=2.17$ if one employs $\Phi(R\approx 0)=1-R^{2}/6$.

\subsection{Virial ratio and instability}\label{sec:Virial}

\hspace{0.6cm}The discussion above lacks the actual argument for the instability problem though, one may not have to resort to the eigenvalue problem based on linear instability;  confinement of the ss-OAFP gas itself may be less sensible as explained below. Figure \ref{Fig.R_PeKeRatio_regVirial}(b) shows the ratio $-\text{PE}/\text{KE}$ regularized by $3/\chi_\text{esc}$, which is a direct graphical representation for the criteria of energy balance in the core (Equation \ref{Eq_crit_neg_PEKE}). That the value reaches unity at $R\approx 0$ implies the validity of the approximation of the DF to $e^{\chi_\text{esc}E}$ at the center of the core (to some extent confirming the correctness of numerical integration). This central behavior and the \emph{low} Virial ratio imply that even the Virial $\mathcal{V}(=-2\text{KE}-\text{PE})$ can be positive. Figure \ref{Fig.R_PeKeRatio_regVirial}(c) shows the Virial regularized by $3PV$; the corresponding mathematical expression is as follows compared to the other models
\begin{align}
\frac{\mathcal{V}}{3PV}=\begin{cases}-1, \hspace{3cm}(\text{IS and polytrope of $m>5$ enclosed by a wall})\\
0, \hspace{3.5cm} (\text{energy-truncated models})\\
0.075 \sim 0.26,   \hspace{1.5cm}(\text{ss-OAFP model})
\end{cases}
\end{align}
As expected, the Virial takes positive values. This would be related to the independence of the core from the inner halo as typically explained \citep[e.g.][]{Lynden_Bell_1968,Cohn_1980}; the ss-OAFP model shows the Virial is not zero but relatively close to zero at the center and $\sim3.5$ times smaller than that for the outer halo (Figure \ref{Fig.R_PeKeRatio_regVirial}(c)). 

Possibility of existence of equilibrium state should be discussed. \citep{Lynden_Bell_1980} suggested for their self-similar gaseous model the gravothermal instability in core collapsing phase could occur if the system was enclosed at radii greater than the radius at which its heat flux is maximized. The discussion above for ss-OAFP model shows, rather, confining the system itself is not possible at any radii to establish equilibrium thermodynamic system due to the high absolute value of total potential energy. The positive Virial implies the confined ss-OAFP model would undergo a global collapse as dense molecular clouds could experience in star formation. To avoid the collapse and achieve an equilibrium state, energy release from binaries and composite system, with e.g. dark matter ( and diffuse gas) to gain positive pressure, may be considered though the both would deepen the central potential due to strong binary energy and dynamical friction on stars respectively even if the pressure in halo is balanced out. Also, the system may be confined by a thermal bath and rubber wall (for change in heat and pressure) or by a wall permeable to particles though, either way due to the negative specific heat or sparse halo the instability and density contrast will be more magnified, as well known that increasing the number of constrains on the equilibrium system, the radius for confinement of self-gravitating system must be smaller. 

The ss-OAFP model is only the case at the \emph{late} stage of core collapse. According to \citep{Cohn_1980}, the characteristics of gravothermal instability appears around at epoch $\chi_\text{esc}\approx 9$ (before the epoch, the system behaves more like a lowered Maxwellian). This implies that at the very center of the system the kernel takes the form $\Omega_\text{tot}\approx e^{9\epsilon}-3e^{9\epsilon}$ in which one must double the first term to calculate the Virial, hence the Vrial is still Positive. One may conclude that the core-collapsing core of isotropic spherical cluster is always unstable or globally collapsing if it is confined by an adiabatic wall due to the deep potential. 







\begin{figure}
	\centering
	\begin{tikzpicture}
	\begin{semilogxaxis}[width=11cm,height=5cm,
	grid=major,ylabel=\Large{$-\frac{2\text{KE}}{\text{PE}}$},xmin=1e-1,xmax=1e18,ymin=0,ymax=1,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=1]{R_Vratio.txt};
      \node[above,black] at (1,0.1) {(a)};
      %\node[above,black] at (0.45,-0.35) {(KMC) };
      %\draw[red,fill=red] (0.446,-0.303) circle;
     %\draw[blue,fill=blue] (0.510,-0.253) circle;
	\end{semilogxaxis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{semilogxaxis}[width=11cm,height=5cm,
	grid=major,ylabel=\Large{$-\frac{\text{3PE}}{\chi_\text{esc}\text{KE}}$},xmin=1e-1,xmax=1e18,ymin=0,ymax=1.2,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=1]{R_PeKeRatio_regVirial.txt};
	\node[above,black] at (1,0.1) {(b)};
	\end{semilogxaxis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{semilogxaxis}[width=11cm,height=5cm,
	grid=major,xlabel=\Large{$R_\text{M}$},ylabel=\Large{$\mathcal{V}/(3PV)$},xmin=1e-1,xmax=1e18,ymin=-0.3,ymax=0,legend pos=south east]
	\addplot [color = red ,mark=no,thick,solid ] table[x index=0, y index=2]{R_PeKeRatio_regVirial.txt};
	\node[above,black] at (1,-0.29) {(c)};
	\end{semilogxaxis}
	\end{tikzpicture}
	\caption{(a) Virial ratio,(b) the ratio of -PE/KE to $\chi_\text{esc}/3$ and (c) the regularized Virial of ss-OAFP model.}
	\label{Fig.R_PeKeRatio_regVirial}
\end{figure}  


